SpatialCoT: Advancing Spatial Reasoning through Coordinate Alignment and Chain-of-Thought for Embodied Task Planning

Spatial reasoning is an essential problem in embodied AI research. Efforts to enhance spatial reasoning abilities through supplementary spatial data and fine-tuning have proven limited and ineffective when addressing complex embodied tasks, largely due to their dependence on language-based outputs. While some approaches have introduced a point-based action space to mitigate this issue, they fall short in managing more intricate tasks within complex environments. This deficiency arises from their failure to fully exploit the inherent thinking and reasoning capabilities that are fundamental strengths of Vision-Language Models (VLMs). To address these limitations, we propose a novel approach named SpatialCoT, specifically designed to bolster the spatial reasoning capabilities of VLMs. Our approach comprises two stages: spatial coordinate bi-directional alignment, which aligns vision-language inputs with spatial coordinates, and chain-of-thought spatial grounding, which harnesses the reasoning capabilities of language models for advanced spatial reasoning. We evaluate SpatialCoT on challenging navigation and manipulation tasks, both in simulation and real-world settings. Experimental results demonstrate that our method significantly outperforms previous state-of-the-art approaches in both tasks.

==> tables/bench_comp.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
Benchmark   & Type                          & Objects & Scenes & Skills \\ \hline
RLBench     & Static Manipulation           &         &        &        \\ \hline
CALVIN      & Static Manipulation           &         &        &        \\ \hline
BEHAVIOR-1K & Mobile Manipulation           &         &        &        \\ \hline
ALFRED      & Mobile Manipulation           &         &        &        \\ \hline
Habitat     & Navigation                    &         &        &        \\ \hline
Ours        & Static \& Mobile Manipulation &         &        &        \\ \hline
\end{tabular}
\end{table*}

==> tables/capabilities.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{c|cc}
\hline
\textbf{Category} & \multicolumn{2}{c}{\textbf{Sub-types}} \\ \hline
\multirow{7}{*}{\textbf{Understanding}} & \multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Object\\ Understanding\end{tabular}}} & Object Position \\ \cline{3-3} 
 & \multicolumn{1}{c|}{} & Object Size \\ \cline{3-3} 
 & \multicolumn{1}{c|}{} & Object Count \\ \cline{3-3} 
 & \multicolumn{1}{c|}{} & Object orientation \\ \cline{2-3} 
 & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Scene\\ Understanding\end{tabular}}} & Functional Understanding \\ \cline{3-3} 
 & \multicolumn{1}{c|}{} & Spatial Relationship (Distance) \\ \cline{3-3} 
 & \multicolumn{1}{c|}{} & Spatial Relationship (Direction) \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Spatial\\ Reasoning\end{tabular}}} & \multicolumn{2}{c}{Spatial Localization prediction} \\ \cline{2-3} 
 & \multicolumn{2}{c}{Object/Scene (partially observed) Prediction} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Spatial-\\ Temporal\\ Reasoning\end{tabular}}} & \multicolumn{2}{c}{Spatial Compatibility} \\ \cline{2-3} 
 & \multicolumn{2}{c}{Affordance Prediction} \\ \cline{2-3} 
 & \multicolumn{2}{c}{Movement/Dynamics Prediction} \\ \hline
\end{tabular}
\label{table:capabilities}
\end{table}

==> tables/end2end_task_planning.tex <==

\begin{table}
\renewcommand{\arraystretch}{1.2}
\centering
\begin{tabular}{c|c|c}
\hline
\textbf{Category} & \textbf{Term} & \textbf{Comment} \\ \hline
\multirow{4}{*}{\textbf{State}} & Visual Occlusion & \begin{tabular}[c]{@{}c@{}}Some objects are obscured\\ by other objects in the\\ current perspective\end{tabular} \\ \cline{2-3} 
 & Stacked Occlusion & \begin{tabular}[c]{@{}c@{}}Occlusion due to stacking\\  between objects\end{tabular} \\ \cline{2-3} 
 & Encased Occlusion & \begin{tabular}[c]{@{}c@{}}Occlusion between objects due \\ to containers (e.g. \\ refrigerators, boxes, etc.)\end{tabular} \\ \cline{2-3} 
 & Objects Properties & \begin{tabular}[c]{@{}c@{}}Variation in object geometry\\ and movable properties\end{tabular} \\ \hline
\multirow{3}{*}{\textbf{Goal}} & Number of Objects & \begin{tabular}[c]{@{}c@{}}Number of objects affects\\  task length and complexity\end{tabular} \\ \cline{2-3} 
 & Spatial Constraints & \begin{tabular}[c]{@{}c@{}}the goal includes some\\  additional spatial contraints\end{tabular} \\ \cline{2-3} 
 & Instruction Abstraction & \begin{tabular}[c]{@{}c@{}}Variation in natural \\ language instruction\end{tabular} \\ \hline
\multirow{2}{*}{\textbf{Action}} & Action Format & \begin{tabular}[c]{@{}c@{}}The format to represent\\  the action\end{tabular} \\ \cline{2-3} 
 & Number of Skills & \begin{tabular}[c]{@{}c@{}}Number of skills to be\\  used in planning\end{tabular} \\ \hline
\textbf{Transition} & Temporal Dependency & xxx \\ \hline
\end{tabular}
\caption{Summary of End-to-end Task Planning}
\end{table}





% \begin{table*}
% \centering
% \begin{tabular}{|>{\raggedright\arraybackslash}m{3cm}|>{\raggedright\arraybackslash}m{3cm}|>{\raggedright\arraybackslash}m{6cm}|>{\raggedright\arraybackslash}m{4cm}|}
% \hline
% \textbf{Category} & \textbf{Term} & \textbf{Summary} & \textbf{Capability} \\
% \hline
% \multirow{3}{*}{\textbf{State Complexity}} 
%     & \textbf{Object Properties} & Variation in object geometry and movable properties. 
%         & Object understanding \\
%     \cline{2-4}
%     & \textbf{Object Layout} & Occlusion and placement inside containers, requiring active perception and commonsense knowledge. 
%         & Object localization \\
%     \cline{2-4}
%     & \textbf{Scene Complexity} & Number of workspaces involved, ranging from single-workspace tasks to multi-room tasks. 
%         & Scene understanding and object relationship understanding \\
% \hline

% \multirow{3}{*}{\textbf{Goal Complexity}} 
%     & \textbf{Object Quantity} & Number of objects affects task length and complexity. 
%         & Temporal reasoning \\
%     \cline{2-4}
%     & \textbf{Spatial Constraints} & Level of precision required for object placement. 
%         & Spatial reasoning \\
%     \cline{2-4}
%     & \textbf{Instruction Complexity} & Variation in natural language instruction specificity. 
%         & Instruction following \\
% \hline

% \multirow{2}{*}{\textbf{Action Complexity}} 
%     & \textbf{Object Ambiguity} & Challenges in identifying the correct object among similar ones. 
%         & Coordinate prediction \\
%     \cline{2-4}
%     & \textbf{Skill Variety} & Different objects and tasks require distinct manipulation and navigation skills. 
%         & Multi-skill agent \\
% \hline

% \multirow{2}{*}{\textbf{Transition}} 
%     & \textbf{Partial observation} &  &\\
%     \cline{2-4}
%     & \textbf{Temporal dependency} &  
%         &  \\
% \hline

% \end{tabular}
% \caption{Summary of Task Complexity Categories, Terms, and Required Capabilities}
% \end{table*}



==> tables/levels.tex <==
\begin{table*}
\centering
\begin{tabular}{|>{\centering\arraybackslash}m{4cm}|>{\centering\arraybackslash}m{2.5cm}|>{\centering\arraybackslash}m{2.5cm}|>{\centering\arraybackslash}m{2.5cm}|>{\centering\arraybackslash}m{2.5cm}|}
\hline
\textbf{Difficulty Level} & \textbf{Occlusion} & \textbf{Stacking} & \textbf{Hinge Objects} & \textbf{Multi-Instances} \\
\hline
\textbf{Level 1} (Easy) & No & No & No & No \\
\hline
\textbf{Level 2} (Moderate) & Yes & No & Yes & No \\
\hline
\textbf{Level 3} (Hard) & Yes & Yes & Yes & No \\
\hline
\textbf{Level 4} (Very Hard) & Yes & Yes & Yes & Yes \\
\hline
\end{tabular}
\caption{Overview of Difficulty Levels and Their Properties}
\end{table*}
